A Vector Potential implementation for Smoothed Particle Magnetohydrodynamics

The development of smooth particle magnetohydrodynamic (SPMHD) has significantly improved the simulation of complex astrophysical processes. However, the preservation the solenoidality of the magnetic field is still a severe problem for the MHD. A formulation of the induction equation with a vector potential would solve the problem. Unfortunately all previous attempts suffered from instabilities. In the present work, we evolve the vector potential in the Coulomb gauge and smooth the derived magnetic field for usage in the momentum equation. With this implementation we could reproduce classical test cases in a stable way. A simple test case demonstrates the possible failure of widely used direct integration of the magnetic field, even with the usage of a divergence cleaning method.

==> Makefile <==
view = 1
latexfile =  rota

deptex = *.tex
##figures = 

TEX = latex

$(latexfile).dvi : $(latexfile).bbl $(deptex) $(latexfile).tex
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
%.eps : %.fig
	fig2dev -L eps $< > $(dir $< )$@

$(latexfile).pdf : $(latexfile).ps
	ps2pdf $(latexfile).ps $(latexfile).pdf

$(latexfile).ps : $(latexfile).dvi
	dvips $(latexfile)

$(latexfile).bbl : $(latexfile).aux
	bibtex $(latexfile).aux
	
$(latexfile).aux :
	latex $(latexfile).tex

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents. 
$(latexfile).tar.gz : *.tex *.bib figure/*
	tar -czvf $(latexfile).tar.gz $^

ps : $(latexfile).ps 

pdf : $(latexfile).pdf

tarball: $(latexfile).tar.gz

#$(latexfile).ps
vps: $(latexfile).ps
	evince -f -p $(view) $(latexfile).ps 

aspell: $(deptex)
	tcsh
	foreach G $(deptex)
	aspell -c -d en $G
	done

clean: 
	rm $(latexfile).dvi 

#do I also delete pdf or ps?

